ClassiFIM: An Unsupervised Method To Detect Phase Transitions

Estimation of the Fisher Information Metric (FIM-estimation) is an important task that arises in unsupervised learning of phase transitions, a problem proposed by physicists. This work completes the definition of the task by defining rigorous evaluation metrics distMSE, distMSEPS, and distRE and introduces ClassiFIM, a novel machine learning method designed to solve the FIM-estimation task. Unlike existing methods for unsupervised learning of phase transitions, ClassiFIM directly estimates a well-defined quantity (the FIM), allowing it to be rigorously compared to any present and future other methods that estimate the same. ClassiFIM transforms a dataset for the FIM-estimation task into a dataset for an auxiliary binary classification task and involves selecting and training a model for the latter. We prove that the output of ClassiFIM approaches the exact FIM in the limit of infinite dataset size and under certain regularity conditions. We implement ClassiFIM on multiple datasets, including datasets describing classical and quantum phase transitions, and find that it achieves a good ground truth approximation with modest computational resources. Furthermore, we independently implement two alternative state-of-the-art methods for unsupervised estimation of phase transition locations on the same datasets and find that ClassiFIM predicts such locations at least as well as these other methods. To emphasize the generality of our method, we also propose and generate the MNIST-CNN dataset, which consists of the output of CNNs trained on MNIST for different hyperparameter choices. Using ClassiFIM on this dataset suggests there is a phase transition in the distribution of image-prediction pairs for CNNs trained on MNIST, demonstrating the broad scope of FIM-estimation beyond physics.

==> Makefile <==
# LaTeX Makefile v0.33 -- LaTeX only
# Based on: https://scaron.info/blog/makefiles-for-latex.html

SHELL := /bin/bash -O nullglob
UNAME := $(shell uname)

TEX_FILES := $(wildcard *.tex)
PDF_FILES := $(TEX_FILES:.tex=.pdf)

ifeq ($(UNAME), Darwin)
    LATEX := pdflatex -interaction=nonstopmode
else
    LATEX := rubber --pdf
endif

.PHONY: all clean

all: $(PDF_FILES)

%.pdf: %.tex $(wildcard *.bib)
	@echo "Compiling $<..."
	@if [ -f $*.aux ]; then bibtex $* || true; fi
	@if [ -f bu1.aux ]; then bibtex bu1 || true; fi
	@if [ -f bu2.aux ]; then bibtex bu2 || true; fi
	$(LATEX) $<

clean:
	@echo "Cleaning up..."
ifeq ($(UNAME), Darwin)
	rm $(foreach file, $(TEX_FILES), $(file:.tex=.{aux,bbl,blg,log,pdf,bcf,nav,out,run.xml,snm,toc,vrb}))
else
	rubber --clean $(TEX_FILES)
endif

WATCH_FILES := *.tex refs.bib *.sty

watch:
	@while true; do \
		if [[ "$(UNAME)" == "Darwin" ]]; then \
			res="$$(fswatch -1 $(WATCH_FILES))"; \
			echo "res:$${res}"; \
		else \
			inotifywait -e modify $(WATCH_FILES); \
		fi; \
		sleep 0.01; \
		make all; \
	done

